Are Large-Language Models Graph Algorithmic Reasoners?

We seek to address a core challenge facing current Large Language Models (LLMs). LLMs have demonstrated superior performance in many tasks, yet continue to struggle with reasoning problems on explicit graphs that require multiple steps. To address this gap, we introduce a novel benchmark designed to evaluate LLM performance on classical algorithmic reasoning tasks on explicit graphs. Our benchmark encompasses five fundamental algorithms: Breadth-First Search (BFS) and Depth-First Search (DFS) for connectivity, Dijkstra's algorithm and Floyd-Warshall algorithm for all nodes shortest path, and Prim's Minimum Spanning Tree (MST-Prim's) algorithm. Through extensive experimentation, we assess the capabilities of state-of-the-art LLMs in executing these algorithms step-by-step and systematically evaluate their performance at each stage. Our findings highlight the persistent challenges LLMs face in this domain and underscore the necessity for advanced prompting techniques and algorithmic instruction to enhance their graph reasoning abilities. This work presents MAGMA, the first comprehensive benchmark focused on LLMs completing classical graph algorithms, and provides a critical step toward understanding and improving their structured problem-solving skills.

==> Figures/Examples/alg_agnostic.tex <==
\begin{figure}
    \begin{tcolorbox}[colback=white!5!white,colframe=blue!75!black,title=1. Connectivity, width=11cm]
        \centerline{\begin{tikzpicture}[every node/.style={circle, draw}]
            % Graph 1
            \node[fill=pink] (1) at (0,0) {1};
            \node (0) at (-1,-1) {0};
            \node (2) at (1,-1) {2};
            \draw (1) -- (0);
            \draw (1) -- (2);
    
            % Graph 2
            \node[fill=pink] (4) at (4,0) {4};
            \node (3) at (3,-1) {3};
            \node (5) at (5,-1) {5};
            \draw (4) -- (3);
            \draw (4) -- (5);
        \end{tikzpicture}}
        \vspace{1em}
        Determine if there is a path between two nodes in the graph. Note that (i,j) means that node i and node j are connected with an undirected edge. Graph: (0,1), (1,2), (3,4), (4,5). \\
        
        \textbf{Q:} Is there a path between node 1 and node 4?
    \end{tcolorbox}

    \begin{tcolorbox}[colback=white!5!white,colframe=green!75!black,title=2. Algorithmic Prompting, width=11cm]
        We can use a \textbf{Depth-First Search (DFS)} algorithm to find the shortest path between two given nodes in an undirected graph. \\
    
        The basic idea is to start at one of the nodes and use DFS to explore all of its adjacent nodes. At each node, you keep track of the distance it takes to reach that node from the starting node. \\
    
        Once you have explored all the adjacent nodes, you can backtrack and pick the node with the shortest distance to the destination node. In an undirected graph, the nodes are numbered from 0 to 4, and the edges are an edge between node 0 and node 4 with weight 4, ... \\
    
        \textbf{Q:} Give the shortest path from node 0 to node 2. \\
        
        \textbf{A:} All the paths from node 0 to node 2 are: \\
        0,3,2 with a total weight of 3+1=4, \\
        0,1,4,2 with a total weight of 3+4+2=9, \\
        0,4,3,2 with a total weight of 4+1+1=6. \\
        The weight of path 0,3,2 is the smallest, so the shortest path from node 0 to node 2 is 0,3,2 with total weight of 4.
    \end{tcolorbox}
\end{figure}

==> Figures/Examples/gpt4_collapse.tex <==
\begin{figure}

    \begin{tcolorbox}[colback=white!10!white,colframe=purple!75!black,title= GPT-4o Collapse Example,sharp corners, box align=top, height=7.00cm, width=\linewidth]
        \textbf{Query:} Please perform the Breadth-first Search algorithm for reachability on the following graph: Edgelist: [((0,2),\textbf{(0,8)},(1,3),(1,4),(1,6),(1,9),(2,5),(2,6),(2,7),(3,4),(3,5),(3,6),(5,6),(5,7),(5,9)]; Source Node: 5; Output Format: Reachable Nodes: [node1, node2, ...]. List all known reachable nodes ordered lexicographically smallest to largest.\\[0.75em]
        \textbf{GPT-4o Response:}\\
        Breadth-first Search (BFS) starting from source node 5:\\
1. Begin at node 5. Add node 5 to the queue and mark it as visited.\\
- Queue: [5]\\
   - Visited: [5]\\
        ...\\
        7. \textbf{Dequeue node 0}. It has \textbf{no unvisited} neighbors.\\
        - Queue: [1]\\
        ...\\
        \textbf{Reachable Nodes}: [5, 2, 6, 7, 9, 0, 1, 3, 4]
        \vspace{2cm}
    \end{tcolorbox}
\end{figure}

==> Tables/0shot_overall.tex <==
% \begin{table}[ht!]
  \caption{Performance comparison of 0-shot SOTA LLM model performance on each algorithm}
  \label{algorithm-comparison}
  \centering
  \begin{tabular}{llcccccc}
    \toprule
    \textbf{Algorithm} & \multirow{2}{*}{\textbf{Prompting Strategy}} & \multicolumn{2}{c}{LLama-2} & \multicolumn{2}{c}{Mistral-2} & \multicolumn{2}{c}{GPT-4} \\
    \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
    & & Acc. & Var. & Acc. & Var. & Acc. & Var. \\
    \midrule
    \multirow{4}{*}{\textbf{Breadth-First Search}}
    & Input-Output      & - & - & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - & - & - \\
    \midrule
    \multirow{4}{*}{\textbf{Depth-First Search}}
    & Input-Output      & - & - & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - & - & - \\
    \midrule
    \multirow{4}{*}{\textbf{Dijkstra's Algorithm}}
    & Input-Output      & - & - & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - & - & - \\
    \midrule
    \multirow{4}{*}{\textbf{Floyd-Warshall Algorithm}}
    & Input-Output      & - & - & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - & - & - \\
    \midrule
    \multirow{4}{*}{\textbf{MST-Prim Algorithm}}
    & Input-Output      & - & - & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - & - & - \\
    \bottomrule
  \end{tabular}
% \end{table}

==> Tables/error_analysis.tex <==
\begin{table*}[ht!]
  \centering
  \small
  \begin{tabular}{llccccc}
    \toprule
    \textbf{Algorithm} & \textbf{Prompt} & \textbf{Model} & \textbf{Missing Prefix} & \textbf{False Neg.} & \textbf{Hallucinations} & \textbf{Invalid Answer Item} \\
    \midrule
    \multirow{4}{*}{BFS} 
      & \multirow{2}{*}{IO} & Llama-3 & 122.0 & 154.69 & 32.46 & 128.31 \\
      & & GPT-4 & 2.69 & 7.08 & 0.0 & 248.77 \\
      & \multirow{2}{*}{Int. Steps} & Llama-3 & 63.69 & 177.23 & 2.46 & 196.15 \\
      & & GPT-4 & 50.85 & 17.31 & 0.23 & 216.85 \\
    \midrule
    \multirow{4}{*}{DFS} 
      & \multirow{2}{*}{IO} & Llama-3 & 69.08 & 564.31 & 515.92 & 202.92 \\
      & & GPT-4 & 46.08 & 650.69 & 535.92 & 209.69 \\
      & \multirow{2}{*}{Int. Steps} & Llama-3 & 69.08 & 564.31 & 515.92 & 202.92 \\
      & & GPT-4 & 58.08 & 582.08 & 525.69 & 220.77 \\
    \midrule
    \multirow{4}{*}{Dijkstra} 
      & \multirow{2}{*}{IO} & Llama-3 & 175.92 & 183.54 & 7.85 & 75.23 \\
      & & GPT-4 & 177.08 & 293.15 & 10.0 & 136.38 \\
      & \multirow{2}{*}{Int. Steps} & Llama-3 & 195.15 & 26.38 & 5.38 & 55.0 \\
      & & GPT-4 & 149.54 & 352.46 & 134.69 & 224.62 \\
    \midrule
    \multirow{4}{*}{Floyd-Warshall} 
      & \multirow{2}{*}{IO} & Llama-3 & 175.58 & 15.58 & 0.83 & 74.5 \\
      & & GPT-4 & 219.15 & 21.23 & 0.08 & 63.08 \\
      & \multirow{2}{*}{Int. Steps} & Llama-3 & 173.31 & 65.38 & 2.85 & 76.69 \\
      & & GPT-4 & 211.92 & 82.77 & 3.23 & 161.23 \\
    \midrule
    \multirow{4}{*}{Prim MST} 
      & \multirow{2}{*}{IO} & Llama-3 & 100.08 & 311.08 & 0.62 & 150.31 \\
      & & GPT-4 & 80.0 & 905.0 & 0.85 & 181.46 \\
      & \multirow{2}{*}{Int. Steps} & Llama-3 & 193.38 & 41.23 & 0.77 & 56.69 \\
      & & GPT-4 & 148.77 & 469.0 & 27.0 & 133.54 \\
    \bottomrule
  \end{tabular}
  \caption{Performance comparison of SOTA LLM model performance in terms of error types on inference trajectories. Lower numbers indicate better performance against a given type of error.}
  \label{error-comparison}
\end{table*}


==> Tables/fewshot_overall.tex <==
% \begin{table}[ht!]
  \caption{Performance comparison of few-shot SOTA LLM model performance on each algorithm}
  \label{algorithm-comparison}
  \centering
  \begin{tabular}{llcccc}
    \toprule
    \textbf{Algorithm} & \multirow{2}{*}{\textbf{Prompting Strategy}} & \multicolumn{2}{c}{LLama-2} & \multicolumn{2}{c}{Mistral-2} \\
    \cmidrule(r){3-4} \cmidrule(r){5-6}
    & & Acc. & Var. & Acc. & Var. \\
    \midrule
    \multirow{4}{*}{\textbf{Breadth-First Search}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - \\
    \midrule
    \multirow{4}{*}{\textbf{Depth-First Search}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - \\
    \midrule
    \multirow{4}{*}{\textbf{Dijkstra's Algorithm}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - \\
    \midrule
    \multirow{4}{*}{\textbf{Floyd-Warshall Algorithm}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - \\
    \midrule
    \multirow{4}{*}{\textbf{MST-Prim Algorithm}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    & Tree-of-Thought   & - & - & - & - \\
    & Graph-of-Thoughts & - & - & - & - \\
    \bottomrule
  \end{tabular}
% \end{table}

==> Tables/finetuned_overall.tex <==
% \begin{table}[ht!]
  \caption{Performance comparison of finetuned LLM model performance on each algorithm}
  \label{algorithm-comparison}
  \centering
  \begin{tabular}{llcccc}
    \toprule
    \textbf{Algorithm} & \multirow{2}{*}{\textbf{Prompting Strategy}} & \multicolumn{2}{c}{LLama-2} & \multicolumn{2}{c}{Mistral-2} \\
    \cmidrule(r){3-4} \cmidrule(r){5-6}
    & & Acc. & Var. & Acc. & Var. \\
    \midrule
    \multirow{2}{*}{\textbf{Breadth-First Search}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    \midrule
    \multirow{2}{*}{\textbf{Depth-First Search}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    \midrule
    \multirow{2}{*}{\textbf{Dijkstra's Algorithm}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    \midrule
    \multirow{2}{*}{\textbf{Floyd-Warshall Algorithm}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    \midrule
    \multirow{2}{*}{\textbf{MST-Prim Algorithm}}
    & Input-Output      & - & - & - & - \\
    & Chain-of-Thought  & - & - & - & - \\
    \bottomrule
  \end{tabular}
% \end{table}

==> Tables/full_FS_EA_table.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Algorithm & Prompting Strategy & Model & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 20 & 50 \\ \hline
Prim's MST & Input-Output (Output + Reasoning) & Mistral-Instruct & 44.00 & 56.00 & 54.00 & 36.00 & 44.00 & 30.00 & 36.00 & 2.00 & 20.00 & 10.00 & 8.00 & 8.03 & 0.00 \\ \hline
Prim's MST & Input-Output (Output + Reasoning) & Mistral & 56.00 & 20.00 & 68.00 & 52.00 & 52.00 & 44.00 & 48.00 & 22.00 & 10.00 & 14.00 & 0.00 & 0.02 & 0.03 \\ \hline
Prim's MST & Input-Output (Output + Reasoning) & Llama-Instruct & 42.86 & 32.80 & 26.00 & 19.60 & 16.80 & 12.40 & 5.20 & 4.00 & 2.00 & 1.20 & 1.20 & 0.40 & 0.00 \\ \hline
Prim's MST & Input-Output (Output + Reasoning) & Llama & 20.00 & 70.00 & 10.00 & 28.00 & 0.00 & 18.00 & 42.00 & 34.00 & 100.00 & 94.00 & 80.00 & 80.04 & 80.06 \\ \hline
Prim's MST & Input-Output (Output + Reasoning) & GPT-4o & 15.18 & 15.20 & 5.60 & 5.60 & 4.00 & 1.60 & 0.80 & 0.00 & 0.80 & 0.11 & 0.20 & 0.00 & 0.00 \\ \hline
Prim's MST & Intermediate Steps & Mistral-Instruct & 66.00 & 56.00 & 56.00 & 66.00 & 48.00 & 0.00 & 42.00 & 38.00 & 84.00 & 62.00 & 54.00 & 53.99 & 50.94 \\ \hline
Prim's MST & Intermediate Steps & Mistral & 68.00 & 44.00 & 66.00 & 48.00 & 62.00 & 0.00 & 38.00 & 46.00 & 12.00 & 50.00 & 48.00 & 40.42 & 37.71 \\ \hline
Prim's MST & Intermediate Steps & Llama-Instruct & 80.00 & 80.00 & 66.00 & 100.00 & 66.00 & 54.00 & 46.00 & 100.00 & 98.00 & 98.00 & 96.00 & 86.00 & 85.19 \\ \hline
Prim's MST & Intermediate Steps & Llama & 82.00 & 80.00 & 68.00 & 98.00 & 48.00 & 0.00 & 46.00 & 74.00 & 96.00 & 100.00 & 100.00 & 94.94 & 91.03 \\ \hline
Prim's MST & Input-Output (Output Only) & Llama-Instruct & 56.00 & 62.00 & 58.00 & 62.00 & 62.00 & 36.00 & 38.00 & 72.00 & 82.00 & 92.00 & 90.00 & 78.00 & 78.00 \\ \hline
Prim's MST & Input-Output (Output Only) & Mistral-Instruct & 72.00 & 72.00 & 58.00 & 46.00 & 56.00 & 80.00 & 66.00 & 32.00 & 74.00 & 54.00 & 72.00 & 61.58 & 61.50 \\ \hline
Prim's MST & Input-Output (Output Only) & Mistral & 68.00 & 42.00 & 72.00 & 40.00 & 58.00 & 72.00 & 72.00 & 46.00 & 18.00 & 56.00 & 76.00 & 69.02 & 68.89 \\ \hline
Prim's MST & Input-Output (Output Only) & Llama-Instruct & 56.25 & 79.20 & 58.40 & 59.20 & 56.00 & 8.80 & 8.40 & 3.60 & 1.60 & 95.20 & 99.20 & 98.80 & 90.64 \\ \hline
Prim's MST & Input-Output (Output Only) & Llama & 80.00 & 80.00 & 72.00 & 64.00 & 0.00 & 98.00 & 98.00 & 42.00 & 100.00 & 100.00 & 100.00 & 93.06 & 93.06 \\ \hline
Floyd-Warshall & Input-Output (Output + Reasoning) & Mistral-Instruct & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 12.00 & 2.00 & 8.00 & 3.21 & 0.00 \\ \hline
Floyd-Warshall & Input-Output (Output + Reasoning) & Mistral & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 14.00 & 4.00 & 8.00 & 7.53 & 4.32 \\ \hline
Floyd-Warshall & Input-Output (Output + Reasoning) & Llama-Instruct & 63.39 & 48.40 & 45.20 & 33.20 & 30.00 & 2.80 & 0.40 & 0.00 & 17.20 & 4.40 & 1.60 & 0.00 & 0.00 \\ \hline
Floyd-Warshall & Input-Output (Output + Reasoning) & Llama & 72.00 & 54.00 & 34.00 & 32.00 & 44.00 & 12.00 & 20.00 & 20.00 & 18.00 & 0.00 & 2.00 & 2.00 & 0.00 \\ \hline
Floyd-Warshall & Input-Output (Output + Reasoning) & GPT-4o & 21.60 & 12.48 & 7.47 & 3.20 & 0.80 & 0.80 & 0.00 & 0.00 & 0.00 & 0.00 & 0.11 & 0.00 & 0.00 \\ \hline
Floyd-Warshall & Intermediate Steps & Mistral-Instruct & 62.00 & 48.00 & 48.00 & 26.00 & 18.00 & 0.00 & 10.00 & 4.00 & 4.00 & 4.00 & 2.00 & 0.28 & 0.00 \\ \hline
Floyd-Warshall & Intermediate Steps & Mistral & 62.00 & 50.00 & 8.00 & 26.00 & 24.00 & 0.00 & 8.00 & 8.00 & 2.00 & 2.00 & 4.00 & 0.00 & 0.00 \\ \hline
Floyd-Warshall & Intermediate Steps & Llama-Instruct & 66.00 & 56.00 & 58.00 & 36.00 & 34.00 & 36.00 & 30.00 & 18.00 & 12.00 & 14.00 & 12.01 & 9.36 & 6.83 \\ \hline
Floyd-Warshall & Intermediate Steps & Llama & 6.00 & 50.00 & 54.00 & 32.00 & 32.00 & 0.00 & 26.00 & 18.00 & 12.00 & 8.00 & 2.00 & 2.00 & 0.53 \\ \hline
Floyd-Warshall & Input-Output (Output Only) & Llama-Instruct & 70.00 & 62.00 & 54.00 & 32.00 & 32.00 & 34.00 & 30.00 & 18.00 & 8.00 & 2.00 & 2.00 & 0.12 & 0.00 \\ \hline
Floyd-Warshall & Input-Output (Output Only) & Mistral-Instruct & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 14.00 & 12.00 & 8.00 & 8.00 & 4.00 & 4.00 & 4.00 & 1.50 \\ \hline
Floyd-Warshall & Input-Output (Output Only) & Mistral & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 8.00 & 8.00 & 10.00 & 8.00 & 2.00 & 0.00 & 0.00 & 0.00 \\ \hline
Floyd-Warshall & Input-Output (Output Only) & Llama-Instruct & 69.64 & 50.40 & 48.00 & 33.20 & 30.40 & 30.80 & 24.40 & 18.80 & 15.20 & 8.80 & 8.80 & 0.00 & 0.00 \\ \hline
Floyd-Warshall & Input-Output (Output Only) & Llama & 12.00 & 52.00 & 52.00 & 40.00 & 46.00 & 18.00 & 28.00 & 20.00 & 18.00 & 6.00 & 2.00 & 2.03 & 0.00 \\ \hline
Dijkstra & Input-Output (Output + Reasoning) & Mistral-Instruct & 68.00 & 74.00 & 54.00 & 54.00 & 12.00 & 60.00 & 28.00 & 28.00 & 12.00 & 30.00 & 30.00 & 25.20 & 25.21 \\ \hline
Dijkstra & Input-Output (Output + Reasoning) & Mistral & 28.00 & 28.00 & 62.00 & 18.00 & 32.00 & 50.00 & 8.00 & 44.00 & 54.00 & 40.00 & 24.00 & 24.16 & 24.28 \\ \hline
Dijkstra & Input-Output (Output + Reasoning) & Llama-Instruct & 31.25 & 35.20 & 22.00 & 29.60 & 24.80 & 12.80 & 12.40 & 8.40 & 2.40 & 4.00 & 2.80 & 1.20 & 0.00 \\ \hline
Dijkstra & Input-Output (Output + Reasoning) & Llama & 4.00 & 34.00 & 0.00 & 66.00 & 0.00 & 28.00 & 30.00 & 14.00 & 84.00 & 72.00 & 76.00 & 75.92 & 63.45 \\ \hline
Dijkstra & Input-Output (Output + Reasoning) & GPT-4o & 36.80 & 30.40 & 32.80 & 25.60 & 20.80 & 16.00 & 7.20 & 6.40 & 2.40 & 0.77 & 0.71 & 0.40 & 0.00 \\ \hline
Dijkstra & Intermediate Steps & Mistral-Instruct & 76.00 & 70.00 & 64.00 & 60.00 & 56.00 & 0.00 & 80.00 & 48.00 & 74.00 & 54.00 & 60.00 & 59.97 & 55.73 \\ \hline
Dijkstra & Intermediate Steps & Mistral & 78.00 & 58.00 & 50.00 & 66.00 & 52.00 & 0.00 & 80.00 & 12.00 & 74.00 & 72.00 & 60.00 & 59.97 & 59.96 \\ \hline
Dijkstra & Intermediate Steps & Llama-Instruct & 78.00 & 70.00 & 66.00 & 94.00 & 66.00 & 50.00 & 96.00 & 98.00 & 100.00 & 100.00 & 100.00 & 86.91 & 86.91 \\ \hline
Dijkstra & Intermediate Steps & Llama & 82.00 & 72.00 & 60.00 & 90.00 & 68.00 & 0.00 & 52.00 & 76.00 & 70.00 & 98.00 & 100.00 & 95.55 & 92.76 \\ \hline
Dijkstra & Input-Output (Output Only) & Llama-Instruct & 78.00 & 80.00 & 68.00 & 98.00 & 62.00 & 54.00 & 98.00 & 92.00 & 96.00 & 100.00 & 100.00 & 93.42 & 93.44 \\ \hline
Dijkstra & Input-Output (Output Only) & Mistral-Instruct & 80.00 & 58.00 & 66.00 & 60.00 & 50.00 & 76.00 & 42.00 & 46.00 & 58.00 & 52.00 & 66.00 & 53.90 & 53.37 \\ \hline
Dijkstra & Input-Output (Output Only) & Mistral & 76.00 & 56.00 & 60.00 & 50.00 & 60.00 & 82.00 & 44.00 & 10.00 & 54.00 & 70.00 & 58.00 & 56.25 & 56.24 \\ \hline
Dijkstra & Input-Output (Output Only) & Llama-Instruct & 41.07 & 50.80 & 25.20 & 23.60 & 15.60 & 8.80 & 10.80 & 7.20 & 2.40 & 4.00 & 1.20 & 0.40 & 0.00 \\ \hline
Dijkstra & Input-Output (Output Only) & Llama & 80.00 & 76.00 & 46.00 & 58.00 & 0.00 & 100.00 & 18.00 & 36.00 & 60.00 & 100.00 & 98.00 & 92.91 & 92.75 \\ \hline
DFS & Input-Output (Output + Reasoning) & Mistral-Instruct & 16.00 & 4.00 & 4.00 & 12.00 & 4.00 & 0.00 & 2.00 & 2.00 & 0.00 & 6.00 & 2.00 & 0.00 & 0.00 \\ \hline
DFS & Input-Output (Output + Reasoning) & Mistral & 8.00 & 12.00 & 0.00 & 2.00 & 0.00 & 0.00 & 6.00 & 2.00 & 2.00 & 4.00 & 4.00 & 0.00 & 0.02 \\ \hline
DFS & Input-Output (Output + Reasoning) & Llama-Instruct & 0.00 & 20.40 & 4.00 & 3.20 & 6.40 & 8.80 & 8.00 & 4.40 & 7.20 & 10.40 & 8.00 & 4.00 & 9.60 \\ \hline
DFS & Input-Output (Output + Reasoning) & Llama & 0.00 & 40.00 & 32.00 & 35.20 & 37.60 & 37.20 & 36.40 & 34.40 & 25.60 & 33.60 & 39.60 & 26.80 & 6.40 \\ \hline
DFS & Input-Output (Output + Reasoning) & GPT-4o & 54.00 & 32.80 & 22.40 & 24.00 & 17.60 & 15.20 & 21.60 & 15.20 & 13.60 & 16.80 & 11.20 & 0.00 & 0.40 \\ \hline
DFS & Intermediate Steps & Mistral-Instruct & 88.00 & 4.00 & 12.00 & 20.00 & 12.00 & 0.00 & 6.00 & 2.00 & 6.00 & 0.00 & 2.00 & 0.00 & 0.00 \\ \hline
DFS & Intermediate Steps & Mistral & 82.00 & 10.00 & 12.00 & 6.00 & 52.00 & 0.00 & 22.00 & 6.00 & 10.00 & 6.00 & 0.00 & 0.13 & 0.20 \\ \hline
DFS & Intermediate Steps & Llama-Instruct & 98.00 & 54.00 & 44.00 & 32.00 & 34.00 & 22.00 & 18.00 & 14.00 & 22.00 & 22.00 & 20.00 & 9.96 & 9.96 \\ \hline
DFS & Intermediate Steps & Llama & 0.00 & 4.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 2.00 & 4.00 & 0.00 & 0.00 & 0.00 \\ \hline
DFS & Input-Output (Output Only) & Llama-Instruct & 94.00 & 48.00 & 58.00 & 26.00 & 68.00 & 72.00 & 68.00 & 32.00 & 24.00 & 18.00 & 12.00 & 12.02 & 12.04 \\ \hline
DFS & Input-Output (Output Only) & Mistral-Instruct & 48.00 & 8.00 & 12.00 & 14.00 & 14.00 & 10.00 & 18.00 & 2.00 & 4.00 & 2.00 & 2.00 & 0.00 & 0.00 \\ \hline
DFS & Input-Output (Output Only) & Mistral & 36.00 & 10.00 & 4.00 & 12.00 & 46.00 & 44.00 & 24.00 & 4.00 & 4.00 & 10.00 & 4.00 & 2.10 & 2.10 \\ \hline
DFS & Input-Output (Output Only) & Llama-Instruct & 0.00 & 1.60 & 5.20 & 4.40 & 6.40 & 9.20 & 7.20 & 5.60 & 10.00 & 2.40 & 2.80 & 0.80 & 0.00 \\ \hline
DFS & Input-Output (Output Only) & Llama & 0.00 & 4.00 & 0.00 & 4.00 & 0.00 & 0.00 & 2.00 & 0.00 & 4.00 & 0.00 & 0.00 & 0.02 & 0.00 \\ \hline
BFS & Input-Output (Output + Reasoning) & Mistral-Instruct & 80.01 & 80.00 & 86.00 & 44.00 & 98.00 & 98.00 & 88.00 & 44.00 & 94.00 & 96.00 & 88.00 & 81.32 & 81.34 \\ \hline
BFS & Input-Output (Output + Reasoning) & Mistral & 66.81 & 74.00 & 82.00 & 44.00 & 64.00 & 74.00 & 22.00 & 70.00 & 10.00 & 30.00 & 70.00 & 65.20 & 59.19 \\ \hline
BFS & Input-Output (Output + Reasoning) & Llama-Instruct & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.20 & 0.00 & 0.80 & 0.00 & 0.00 & 0.40 & 64.00 \\ \hline
BFS & Input-Output (Output + Reasoning) & Llama & 8.00 & 26.00 & 30.00 & 0.00 & 0.00 & 22.00 & 0.00 & 26.00 & 86.00 & 98.00 & 4.00 & 4.00 & 4.00 \\ \hline
BFS & Input-Output (Output + Reasoning) & GPT-4o & 36.36 & 31.20 & 29.60 & 30.40 & 34.40 & 31.20 & 34.40 & 32.00 & 19.20 & 20.80 & 24.80 & 2.01 & 0.00 \\ \hline
BFS & Intermediate Steps & Mistral-Instruct & 72.00 & 86.00 & 32.00 & 28.00 & 26.00 & 0.00 & 78.00 & 80.00 & 70.00 & 88.00 & 94.00 & 92.70 & 84.25 \\ \hline
BFS & Intermediate Steps & Mistral & 30.00 & 94.00 & 40.00 & 72.00 & 40.00 & 0.00 & 78.00 & 90.00 & 88.00 & 50.00 & 2.00 & 2.28 & 2.48 \\ \hline
BFS & Intermediate Steps & Llama-Instruct & 96.00 & 100.00 & 76.00 & 94.00 & 62.00 & 94.00 & 100.00 & 98.00 & 98.00 & 88.00 & 46.00 & 46.03 & 46.05 \\ \hline
BFS & Intermediate Steps & Llama & 0.00 & 0.00 & 28.00 & 24.00 & 22.00 & 0.00 & 96.00 & 20.00 & 6.00 & 46.00 & 66.00 & 57.34 & 52.89 \\ \hline
BFS & Input-Output (Output Only) & Llama-Instruct & 98.00 & 100.00 & 72.00 & 94.00 & 52.00 & 90.00 & 94.00 & 98.00 & 96.00 & 92.00 & 100.00 & 96.40 & 86.23 \\ \hline
BFS & Input-Output (Output Only) & Mistral-Instruct & 0.00 & 52.00 & 54.00 & 8.00 & 32.00 & 52.00 & 66.00 & 86.00 & 80.00 & 86.00 & 86.00 & 80.66 & 71.37 \\ \hline
BFS & Input-Output (Output Only) & Mistral & 20.00 & 84.00 & 62.00 & 42.00 & 40.00 & 62.00 & 78.00 & 92.00 & 96.00 & 70.00 & 0.00 & 0.09 & 0.15 \\ \hline
BFS & Input-Output (Output Only) & Llama-Instruct & 70.58 & 73.20 & 74.40 & 72.80 & 64.00 & 50.00 & 60.80 & 69.20 & 54.00 & 63.20 & 51.20 & 27.20 & 82.00 \\ \hline
BFS & Input-Output (Output Only) & Llama & 4.00 & 0.00 & 54.00 & 10.00 & 28.00 & 8.00 & 94.00 & 14.00 & 6.00 & 58.00 & 62.00 & 49.14 & 49.31 \\ \hline
\end{tabular}}
\caption{Full Final Step Exact Accuracy Results}
\end{table*}


==> Tables/overall.tex <==
\newcommand{\bc}[1]{\underline{\textbf{#1}}}

\begin{table*}[ht!]
  \centering
  \resizebox{\linewidth}{!}{
  \small
  \begin{tabular}{llcccccccccccccc}
    \toprule
    \textbf{Algorithm} & \textbf{Prompt} & \textbf{Model} & \multicolumn{13}{c}{Graph Size} \\
    \cmidrule(r){4-16}
    & & & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 20 & 50 \\
    \midrule
    \multirow{4}{*}{BFS} & \multirow{2}{*}{IO} & Llama-3 & \underline{0.33} & \bc{0.41} & \bc{0.46} & \bc{0.45} & \bc{0.37} & \underline{0.27} & \bc{0.32} & \underline{0.32} & \underline{0.26} & \underline{0.30} & \underline{0.23} & \underline{0.12} & \underline{0.32} \\
    & & GPT-4 & 0.27 & 0.23 & 0.24 & 0.19 & 0.16 & 0.19 & 0.07 & 0.07 & 0.09 & 0.07 & 0.06 & 0.05 & 0.20 \\
    & \multirow{2}{*}{Int. Steps} & Llama-3 & \bc{0.41} & \underline{0.28} & \underline{0.27} & \underline{0.27} & 0.25 & \bc{0.36} & 0.22 & \bc{0.34} & \bc{0.29} & \bc{0.43} & \bc{0.42} & \bc{0.27} & \bc{0.39} \\
    & & GPT-4 & \bc{0.41} & 0.21 & \underline{0.27} & 0.24 & \underline{0.32} & 0.25 & \underline{0.28} & 0.29 & 0.26 & 0.19 & 0.13 & 0.10 & 0.24 \\
    \midrule
    \multirow{4}{*}{DFS} & \multirow{2}{*}{IO} & Llama-3 & 0.59 & \bc{0.63} & \underline{0.22} & 0.20 & 0.20 & \underline{0.11} & 0.14 & 0.14 & \bc{0.23} & \bc{0.25} & 0.25 & \bc{0.36} & \bc{0.38} \\
    & & GPT-4 & \bc{0.63} & 0.24 & 0.08 & \bc{0.25} & \bc{0.35} & 0.06 & \bc{0.35} & \underline{0.22} & 0.12 & 0.13 & \bc{0.26} & 0.14 & 0.07 \\
    & \multirow{2}{*}{Int. Steps} & Llama-3 & 0.57 & 0.25 & 0.11 & 0.16 & \underline{0.07} & 0.11 & \underline{0.26} & \bc{0.23} & \underline{0.18} & \underline{0.13} & 0.12 & \underline{0.14} & \underline{0.07} \\
    & & GPT-4 & \underline{0.58} & \underline{0.27} & \bc{0.24} & \underline{0.20} & 0.06 & \bc{0.13} & 0.16 & 0.22 & 0.15 & 0.11 & \bc{0.26} & 0.11 & \underline{0.07} \\
    \midrule
    \multirow{4}{*}{Dijkstra} & \multirow{2}{*}{IO} & Llama-3 & \bc{0.34} & \bc{0.38} & \underline{0.23} & \underline{0.22} & \underline{0.17} & \underline{0.10} & \underline{0.11} & \underline{0.10} & \underline{0.09} & \underline{0.07} & \underline{0.07} & \underline{0.05} & \underline{0.04} \\
    & & GPT-4 & 0.09 & 0.05 & 0.07 & 0.04 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.03 \\
    & \multirow{2}{*}{Int. Steps} & Llama-3 & 0.29 & \underline{0.35} & 0.25 & \bc{0.27} & 0.25 & \bc{0.36} & 0.22 & \bc{0.34} & \bc{0.29} & \bc{0.43} & \bc{0.42} & \bc{0.27} & \bc{0.39} \\
    & & GPT-4 & \underline{0.31} & 0.21 & \bc{0.27} & 0.24 & \bc{0.32} & 0.25 & \bc{0.28} & 0.29 & 0.26 & 0.19 & 0.13 & 0.10 & 0.24 \\
    \midrule
    \multirow{4}{*}{Floyd-Warshall} & \multirow{2}{*}{IO} & Llama-3 & \bc{0.57} & \bc{0.43} & \bc{0.51} & \bc{0.45} & \bc{0.40} & \underline{0.30} & \underline{0.40} & \underline{0.30} & \underline{0.25} & \underline{0.23} & \underline{0.20} & \underline{0.15} & \underline{0.10} \\
    & & GPT-4 & 0.00 & 0.01 & 0.04 & 0.02 & 0.07 & 0.04 & 0.00 & 0.06 & 0.04 & 0.06 & 0.00 & 0.03 & 0.02 \\
    & \multirow{2}{*}{Int. Steps} & Llama-3 & \underline{0.53} & \underline{0.41} & \underline{0.47} & \underline{0.40} & \underline{0.38} & \bc{0.31} & \bc{0.32} & \bc{0.32} & \bc{0.28} & \bc{0.25} & \bc{0.22} & \bc{0.16} & \bc{0.11} \\
    & & GPT-4 & 0.10 & 0.12 & 0.09 & 0.08 & 0.11 & 0.07 & 0.09 & 0.10 & 0.08 & 0.11 & 0.12 & 0.10 & 0.09 \\
    \midrule
    \multirow{4}{*}{Prim MST} & \multirow{2}{*}{IO} & Llama-3 & \bc{0.41} & \bc{0.45} & \bc{0.47} & \bc{0.51} & \bc{0.43} & \bc{0.39} & \bc{0.36} & \bc{0.32} & \bc{0.35} & \bc{0.37} & \bc{0.32} & \bc{0.35} & \bc{0.39} \\
    & & GPT-4 & 0.11 & 0.09 & 0.07 & 0.04 & 0.03 & 0.06 & 0.05 & 0.04 & 0.02 & 0.03 & 0.03 & 0.02 & 0.01 \\
    & \multirow{2}{*}{Int. Steps} & Llama-3 & \underline{0.24} & \underline{0.18} & \underline{0.15} & \underline{0.08} & 0.08 & \underline{0.06} & \underline{0.03} & \underline{0.04} & \underline{0.03} & \underline{0.03} & \underline{0.02} & \underline{0.02} & \underline{0.05} \\
    & & GPT-4 & 0.11 & 0.14 & 0.05 & 0.02 & \underline{0.10} & 0.04 & \underline{0.03} & 0.03 & \underline{0.03} & 0.01 & \underline{0.02} & 0.01 & 0.03 \\
    \bottomrule
  \end{tabular}
  }
  \caption{Performance comparison of SOTA LLM model performance. Llama-3 models are finetuned prior to inference and GPT-4o models are 0-shot. \textbf{Bold} indicates the best model for a specific graph size for an algorithm. \underline{Underline} indicates the better model using the same prompting strategy.}
  \label{algorithm-comparison}
\end{table*}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

